Multi-granularity for knowledge distillation

Considering the fact that students have different abilities to understand the knowledge imparted by teachers, a multi-granularity distillation mechanism is proposed for transferring more understandable knowledge for student networks. A multi-granularity self-analyzing module of the teacher network is designed, which enables the student network to learn knowledge from different teaching patterns. Furthermore, a stable excitation scheme is proposed for robust supervision for the student training. The proposed distillation mechanism can be embedded into different distillation frameworks, which are taken as baselines. Experiments show the mechanism improves the accuracy by 0.58% on average and by 1.08% in the best over the baselines, which makes its performance superior to the state-of-the-arts. It is also exploited that the student's ability of fine-tuning and robustness to noisy inputs can be improved via the proposed mechanism. The code is available at https://github.com/shaoeric/multi-granularity-distillation.

==> tables/table_model_complexity.tex <==
\begin{table}[htbp]
	\centering
	\caption{Model complexity on the CIFAR100 dataset.}
	\label{Model complexity}
	\begin{tabular}{ccc}
		\toprule
		model       & FLOPs    & params \\ \midrule
		MobileNetV2 & 6.94M    & 0.81M  \\
		ShuffleV1   & 40.45M   & 0.94M  \\
		resnet20    & 41.22M   & 0.27M  \\
		resnet32    & 69.76M   & 0.47M  \\
		resnet56    & 126.84M  & 0.86M  \\
		resnet110   & 255.27M  & 1.73M  \\
		wrn16\_2    & 101.61M  & 0.70M  \\
		wrn40\_1    & 84.00M   & 0.57M  \\
		wrn40\_2    & 329.02M  & 2.25M  \\
		resnet8x4   & 177.82M  & 1.23M  \\
		resnet34x4  & 1085.63M & 7.43M  \\
		vgg8        & 96.59M   & 3.96M  \\
		vgg13       & 285.73M  & 9.46M  \\ \bottomrule
	\end{tabular}
\end{table}
